Many-Body Coarse-Grained Interactions using Gaussian Approximation Potentials

This thesis introduces a framework that is able to describe general many-body coarse-grained interactions. We make use of this to describe the free energy surface as a cluster expansion in terms of monomer, dimer, and trimer terms. The contributions to the free energy due to these terms are inferred from MD results of the underlying all-atom model using Gaussian Approximation Potentials, a type of machine-learning potential based on Gaussian process regression. This provides CG interactions that are much more accurate than is possible with site-based pair potentials. While slower than these, it can still be faster than all-atom simulations for solvent-free CG models of systems with a large amount of solvent, as is common in biomolecular simulations.

==> titlepage.tex <==
%%%%% Title page

%XXX \todo{fix geometry?}

\pagestyle{empty}
\begin{center}
  \Huge

  \makeatletter
  \@title\\
  \makeatother

  \vspace*{1.5cm}
  \includegraphics[width=0.35\textwidth]{cam-crest.pdf}
  \vspace*{1.5cm}
  \huge
  \vspace*{0.5cm}

  \makeatletter
  \@author
  \makeatother

  \vspace{1.5cm}
  \LARGE
  Peterhouse\\
  \Large
  September 2016\\
  \vspace{1.5cm}
  This dissertation is submitted for the degree of\\Doctor of Philosophy.
\end{center}

\cleardoublepage

